Interference Mitigation via Interference-Aware Successive Decoding

In modern wireless networks, interference is no longer negligible since each cell becomes smaller to support high throughput. The reduced size of each cell forces to install many cells, and consequently causes to increase inter-cell interference at many cell edge areas. This paper considers a practical way of mitigating interference at the receiver equipped with multiple antennas in interference channels. Recently, it is shown that the capacity region of interference channels over point-to-point codes could be established with a combination of two schemes: treating interference as noise and jointly decoding both desired and interference signals. In practice, the first scheme is straightforwardly implementable, but the second scheme needs impractically huge computational burden at the receiver. Within a practical range of complexity, this paper proposes the interference-aware successive decoding (IASD) algorithm which successively decodes desired and interference signals while updating a priori information of both signals. When multiple decoders are allowed to be used, the proposed IASD can be extended to interference-aware parallel decoding (IAPD). The proposed algorithm is analyzed with extrinsic information transfer (EXIT) chart so as to show that the interference decoding is advantageous to improve the performance. Simulation results demonstrate that the proposed algorithm significantly outperforms interference non-decoding algorithms.

==> background.tex <==
\subsection{Interference Channel}

\subsection{Achievable Rate Region}
